DOTA: Distributional Test-Time Adaptation of Vision-Language Models

Vision-language foundation models (VLMs), such as CLIP, exhibit remarkable performance across a wide range of tasks. However, deploying these models can be unreliable when significant distribution gaps exist between training and test data, while fine-tuning for diverse scenarios is often costly. Cache-based test-time adapters offer an efficient alternative by storing representative test samples to guide subsequent classifications. Yet, these methods typically employ naive cache management with limited capacity, leading to severe catastrophic forgetting when samples are inevitably dropped during updates. In this paper, we propose DOTA (DistributiOnal Test-time Adaptation), a simple yet effective method addressing this limitation. Crucially, instead of merely memorizing individual test samples, DOTA continuously estimates the underlying distribution of the test data stream. Test-time posterior probabilities are then computed using these dynamically estimated distributions via Bayes' theorem for adaptation. This distribution-centric approach enables the model to continually learn and adapt to the deployment environment. Extensive experiments validate that DOTA significantly mitigates forgetting and achieves state-of-the-art performance compared to existing methods.

==> tables/ablation_ood_mean_placements.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand\arraystretch{0.95}
\begin{table*}[!ht]
  \centering
  \resizebox{\linewidth}{!}{
\begin{tabular}{l*{11}c}
  \toprule
   {Method}    &  ImageNet   &  ImageNet-A  &  ImageNet-V2  & ImageNet-R & ImageNet-S  &Average      \\
  \midrule
  \cta  & 70.68 & 61.19 & 64.41 & 81.17 & 51.33 & 65.77 \\
  \midrule
  \multirow{2}{*}{w/o covariance} & 69.62 & 60.29 & 64.15 & 80.21 & 50.42 & 64.94 \\
   &  \textcolor{brown}{-1.06}  &  \textcolor{brown}{-0.90}  &  \textcolor{brown}{-0.26}  &  \textcolor{brown}{-0.96}  &  \textcolor{brown}{-0.91}  & \textcolor{brown}{-0.83}  \\
    \bottomrule
\end{tabular}
}
  \caption{Ablation study comparing the performance of \cta with a variant that uses only the mean, excluding the estimation of the Gaussian distribution (by removing the covariance matrix).}
  % The third row highlights the extent of accuracy reduction.}
  \label{tab:ablation_ood_mean_placements}
  % \vspace{10pt}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
  

==> tables/fine_grained_improvements.tex <==
\begin{table*}[!h]
  \centering
  \resizebox{\linewidth}{!}{
    % 第二个表格
    \begin{tabular}{c|*{11}c>{\columncolor{gray!10}}c}
      \toprule
      Feedback  Percentile & Method & Aircraft & Caltech101 & Cars & DTD & EuroSAT & Flower102 & Food101 & Pets & SUN397 & UCF101 & Average \\
      \midrule
      % \rowcolor{gray!10} 
       \cellcolor{white}\multirow{3}{*}{{5\%}} &{Random} & 26.58 & 94.36 & 70.22 & 48.94 & 65.25 & 75.48 & 87.08 & 92.07 & 70.18 & 73.43 & {70.36}  \\
    
       & {Similarity} & 27.06 & 94.36 & 70.30  & 50.24 & 63.38 & 76.17 & 87.11 & 92.42 & 70.28 & 74.41 & {70.57} \\
       & {Confidence} & 26.73 & 94.56 & 70.95 & 49.82 & 65.00    & 76.86 & 87.17 & 92.78 & 70.49 & 75.26 & {70.96} \\
      \midrule
      % \rowcolor{gray!10} 
       \cellcolor{white}\multirow{3}{*}{{15\%}} & {Random} & 28.68 & 94.69 & 71.57 & 50.83 & 74.63 & 76.37 & 87.15 & 92.34 & 70.93 & 75.71 & {72.29}  \\
    
      & {Similarity} & 29.46 & 94.56 & 72.27 & 53.84 & 71.09 & 78.97 & 87.24 & 93.08 & 71.42 & 76.55 & {72.85}  \\
      & {Confidence} & 28.65 & 95.01 & 73.01 & 53.78 & 76.60  & 79.70  & 87.41 & 93.54 & 71.82 & 79.33 & {73.89} \\
      \bottomrule
    \end{tabular}
}
\caption{Top-1 accuracy (\%) of experimental results using the ViT-B/16 backbone with different methods for selecting uncertainty samples for human feedback. Random, Similarity, and Confidence refer to Randomly selecting inference samples, selecting based on zero-shot cosine similarity, and selecting based on the confidence of the zero-shot classifier, respectively.}
\label{tab:ablation_uncertainty}
\end{table*}

==> tables/fine_grained_strategies.tex <==
\begin{table*}[!h]
  \centering
%   \resizebox{\linewidth}{!}{
%     % 第二个表格
%     \begin{tabular}{c|*{12}c}
    
%       \toprule
%       Feedback Percentile & Method  & ImageNet   &  ImageNet-A  &  ImageNet-V2  & ImageNet-R 
%     & ImageNet-S   
%     & Average      \\
%       \midrule
%       \rowcolor{gray!15} 
%        \cellcolor{white}\multirow{3}{*}{{5\%}} &{random} & 68.78 & 59.94 & 64.17 & 80.44 & 49.42 & {64.55}\textit{(bs)}  \\
%        & {Similarity} &  42.10  & 33.66 & 34.76 & 36.78 & 16.07 & {32.67}{\small (31.88\textcolor{ red}{$\downarrow$})} \\
%        & {Confidence} &19.85 & 21.56 & 17.63 & 21.23 & 6.59  & {17.37}{\small (47.18\textcolor{ red}{$\downarrow$})} \\
%       \midrule
%       \rowcolor{gray!15} 
%        \cellcolor{white}\multirow{3}{*}{{15\%}} & {random} & 68.78 & 59.94 & 64.17 & 80.44 & 49.42 & {64.55}\textit{(bs)} \\
    
%       & {Similarity} & 48.91 & 36.35 & 39.46 & 47.09 & 21.42 & {38.65}{\small (25.90\textcolor{ red}{$\downarrow$})} \\
%       & {Confidence} &28.84 & 27.07 & 25.50  & 35.96 & 11.82 & {25.84}{\small (38.71\textcolor{ red}{$\downarrow$})}\\
%       \bottomrule
%     \end{tabular}
% }  
  \resizebox{\linewidth}{!}{
    % 第二个表格
    \begin{tabular}{c|*{11}c>{\columncolor{gray!10}}c}
      \toprule
      Feedback Percentile & Method & Aircraft & Caltech101 & Cars & DTD & EuroSAT & Flower102 & Food101 & Pets & SUN397 & UCF101 & Average \\
      \midrule
      \rowcolor{gray!15} - & Baseline & 23.22  & 93.55  & 66.11  & 45.04  & 50.42  & 66.99  & 82.86  & 86.92  & 65.63  & 65.16  & 64.59  \\
      \midrule
    
       \cellcolor{white}\multirow{2}{*}{{5\%}} & {Similarity} & 19.32 & 91.95 & 51.76 & 30.36 & 5.00     & 42.86 & 54.56 & 50.00    & 55.61 & 32.22  & {43.36}\\
   
       & {Confidence} & 11.80  & 68.35 & 25.00    & 15.87 & 20.51 & 9.63  & 31.74 & 37.93 & 19.79 & 18.09  & {25.87}\\
      \midrule
      % \rowcolor{gray!15} 
       % \cellcolor{white}\multirow{3}{*}{{15\%}} & {random} & 24.66 & 94.30  & 65.93 & 44.59 & 48.22 & 70.12 & 85.91 & 88.59 & 66.98 & 65.75 & {65.51}\textit{(bs)} \\
    
    \cellcolor{white}\multirow{2}{*}{{15\%}}  & {Similarity} & 21.37 & 95.74 & 58.94 & 32.70  & 13.73 & 37.89 & 63.40  & 65.74 & 55.91 & 45.68 & {49.11}\\
      & {Confidence} & 11.36 & 71.81 & 29.81 & 18.12 & 19.63 & 20.16 & 44.91 & 52.04 & 30.66 & 21.42  & {31.99}\\
      \bottomrule
    \end{tabular}
}
\caption{Top-1 accuracy (\%) of uncertainty samples selected by different methods. `Baseline' indicates the original zero-shot classification results. Lower accuracy suggests better identification of uncertain samples by the method.}
\label{tab:uncertainsampleacc}
\end{table*}
  




==> tables/imagenetv2.tex <==
\begin{table}[!h] % 右侧浮动，宽度为文本宽度的一半
  \caption{Comparisons of our \cta with other methods on the ImageNetV2 dataset, where each class contains only 10 samples. }
  \centering
  \resizebox{0.45\linewidth}{!}{ % 将宽度设置为原始宽度的 90%
    \begin{tabular}{lccc}
      \toprule % 添加表格的上边线
      Method & ViT-B/16 & ResNet-50  \\ \midrule
      \rowcolor{gray!10}  Zero-Shot & 61.88 & 52.91\\
     \midrule
      % TPT & 63.45 & 54.70  \\
      % DiffTPT & 65.10 & 55.80  \\
      TDA & 64.67 & 55.54 \\
      \cta (All test samples) & 64.50 & 55.19 \\ 
\cta (last 50\% test samples ) & 65.20 & 55.72 \\ 
      \bottomrule
    \end{tabular}
  }
  \label{tab:imagenetv2}
\end{table}

==> tables/medical_plip.tex <==
% \begin{table}[h!]
% \caption{Performance comparison across datasets on PLIP model.}
% \centering
% \resizebox{0.7\linewidth}{!}{
% \begin{tabular}{clccccc}
% \toprule
% Model & Dataset          & Kather & PanNuke & WSSS4LUAD & Average \\ 
% \midrule
% \multirow{3}{*}{\rotatebox{90}{PLIP}} & Zero-Shot  & 45.60  & 69.49 & 70.31 & 61.80 \\
% & TDA              &49.35 & 69.70  & 71.96 & 63.67 \\
% & \cta             & 61.92 & 74.68 & 75.07 & 70.56 \\
% % \multirow{3}{*}{\rotatebox{90}{PLIP}} & Zero-Shot  & 45.60  & 71.56   & 70.31     & 62.49   \\
% % & TDA              & 49.39  & 71.56   & 72.13     & 64.36   \\
% % & DOTA             & 55.22  & 72.25   & 72.32     & 66.60   \\ 
% \bottomrule
% \end{tabular}
% }
% \label{tab:dataset_comparison_plip}
% \end{table}


\begin{table}[h!]
\caption{Performance comparison across datasets on PLIP model.}
\centering
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{cccc}
\toprule
{Dataset} & {Zero-Shot} & {TDA} & {CTA} \\
\hline
{Kather} & 45.60 & 49.35 & 61.92 \\
PanNuke & 69.49 & 69.70 & 74.68 \\
WSSS4LUAD & 70.31 & 71.96 & 75.07 \\
average & 61.80& 63.67 & 70.56\\
\bottomrule
\end{tabular}
}
\label{tab:dataset_comparison_plip}
\end{table}


==> tables/ood_improments.tex <==
\begin{table*}[ht]
  \centering
  \resizebox{\linewidth}{!}{
    % 第二个表格
    
    \begin{tabular}{c|*{12}c}
    
      \toprule
      Feedback Percentile & Method  & ImageNet   &  ImageNet-A  &  ImageNet-V2  & ImageNet-R 
    & ImageNet-S   
    & Average      \\
      \midrule
      \rowcolor{gray!15} 
       \cellcolor{white}\multirow{3}{*}{\textbf{5\%}} &\textbf{random} & 70.86 & 61.53 & 64.39 & 81.28 & 51.83 & \textbf{65.98}\textit{(bs)} \\
       & \textbf{max\_logit} &  71.11 & 61.40  & 64.26 & 81.43 & 51.58 & \textbf{65.96}{\small (-0.02)} \\
       & \textbf{softmax} &71.01 & 61.44 & 64.45 & 81.41 & 52.13 & \textbf{66.09}{\small (+0.11)} \\
      \midrule
      \rowcolor{gray!15} 
       \cellcolor{white}\multirow{3}{*}{\textbf{15\%}} & \textbf{random} & 71.28 & 61.79 & 64.59 & 81.39 & 52.75 & \textbf{66.36}\textit{(bs)} \\
    
      & \textbf{max\_logit} & 71.68 & 61.77 & 64.39 & 81.77 & 52.77 & \textbf{66.48}{\small (+0.12)} \\
      & \textbf{softmax} & 71.83 & 61.83 & 64.53 & 81.78 & 53.34 & \textbf{66.66}{\small (+0.30)} \\
      \bottomrule
    \end{tabular}
}
\caption{\textbf{Results on the OOD Benchmark}. 
}
\label{tab:ood-improvements}
\end{table*}

==> tables/ood_strategies.tex <==
\begin{table*}[ht]
  \centering
  \resizebox{\linewidth}{!}{
    % 第二个表格
    
    \begin{tabular}{c|*{12}c}
    
      \toprule
      Feedback Percentile & Method  & ImageNet   &  ImageNet-A  &  ImageNet-V2  & ImageNet-R 
    & ImageNet-S   
    & Average      \\
      \midrule
      \rowcolor{gray!15} 
       \cellcolor{white}\multirow{3}{*}{\textbf{5\%}} &\textbf{random} & 68.78 & 59.94 & 64.17 & 80.44 & 49.42 & \textbf{64.55}\textit{(bs)}  \\
       & \textbf{max\_logit} &  42.10  & 33.66 & 34.76 & 36.78 & 16.07 & \textbf{32.67}{\small (31.88\textcolor{ red}{$\downarrow$})} \\
       & \textbf{softmax} &19.85 & 21.56 & 17.63 & 21.23 & 6.59  & \textbf{17.37}{\small (47.18\textcolor{ red}{$\downarrow$})} \\
      \midrule
      \rowcolor{gray!15} 
       \cellcolor{white}\multirow{3}{*}{\textbf{15\%}} & \textbf{random} & 68.78 & 59.94 & 64.17 & 80.44 & 49.42 & \textbf{64.55}\textit{(bs)} \\
    
      & \textbf{max\_logit} & 48.91 & 36.35 & 39.46 & 47.09 & 21.42 & \textbf{38.65}{\small (25.90\textcolor{ red}{$\downarrow$})} \\
      & \textbf{softmax} &28.84 & 27.07 & 25.50  & 35.96 & 11.82 & \textbf{25.84}{\small (38.71\textcolor{ red}{$\downarrow$})}\\
      \bottomrule
    \end{tabular}
}
\caption{\textbf{Results on the OOD Benchmark}. 
}
\label{tab:ood-strategies}
\end{table*}
